AntiCopyPaster 2.0: Whitebox just-in-time code duplicates extraction

AntiCopyPaster is an IntelliJ IDEA plugin, implemented to detect and refactor duplicate code interactively as soon as a duplicate is introduced. The plugin only recommends the extraction of a duplicate when it is worth it. In contrast to current Extract Method refactoring approaches, our tool seamlessly integrates with the developer's workflow and actively provides recommendations for refactorings. This work extends our tool to allow developers to customize the detection rules, i.e., metrics, based on their needs and preferences. The plugin and its source code are publicly available on GitHub at https://github.com/refactorings/anti-copy-paster. The demonstration video can be found on YouTube: https://youtu.be/ Y1sbfpds2Ms.

==> figures/Usefulness.tex <==
\begin{figure}[h]  
\centering 
\begin{tikzpicture}
\begin{scope}[scale=0.5]
\begin{axis}[
    ybar stacked,
    height=11cm,
    width=10cm,
   % percentage plot,
    bar width=0.80cm, % increased from 0.3cm
    xticklabels from table={\dataA}{Category}, % read ticklabels from first column
    xtick=data,
    x tick label style={
      rotate=45,
      anchor=east, 
      xshift=-1.5mm, yshift=-2mm
    },
    legend style={
      at={(0.5,-0.3)},
      anchor=south,
      legend columns=-1
      },
]

    %\addplot [fill=red!60]  table[percentage series=1] {\dataA};
    %\addplot [fill=orange!60]                 table[percentage series=2] {\dataA};
    \addplot [fill=yellow!60]       table[percentage series=1] {\dataA};
    \addplot [fill=cyan!60]       table[percentage series=2] {\dataA};
    \addplot [fill=blue!60]       table[percentage series=3] {\dataA};
    \addplot [fill=red!60]       table[percentage series=4] {\dataA};
    \addplot [fill=orange!60]       table[percentage series=5] {\dataA};
    % plot just to add total
    %\addplot [forget plot,nodes near coords align=above] table[x expr=\coordindex,y expr=0.0001,meta=sum]{\dataA};

    \legend{\strut Very Satisfied, \strut Somewhat Satisfied, \strut Neural, \strut Somewhat Unsatisfied, \strut Very Unsatisfied}
\end{axis}
\end{scope}
\end{tikzpicture}
\caption{Participants’ satisfaction with various aspects of
the \toolname tool}
\label{fig:usefulness}
\end{figure}

==> sections/05-conclusion.tex <==
\section{Conclusion}
Recommending \textit{Extract Method} refactoring possibilities is of significant importance for the research community and the industry. In this study, we introduced an extension to the \toolname tool, which functions as an IntelliJ IDEA plugin. Our investigation centered on allowing developers to tailor the detection rules (\ie metrics), according to their individual needs and preferences.
%In the future, we plan to add support for other programming languages that could expand the utility of the plugin. Another potential upgrade is to use artificial intelligence to suggest names for extracted methods based on duplicate code. 
%Recommending \textit{Extract Method} refactoring opportunities is critical to both the research community and industry. Despite the fact that numerous research works have used a number of ways to discover \textit{Extract Method} refactoring, advocating this refactoring type without interfering with developers' workflow has largely remained unexplored. In this study, we proposed \toolname as an IntelliJ IDEA plugin, and experimented with machine learning models in order to increase the adoption and usage of the \textit{Extract Method} refactoring while maintaining the workflow of a developer. Our findings show that machine learning models are efficient in identifying \textit{Extract Method} refactoring opportunities as soon as code duplicates are presented in the IDE, and that the \toolname tool was well received by developers.


==> tables/results.tex <==
\begin{table}[]
\begin{center}
\caption{The performance of different classifiers.}
\label{Table:binary_classifiers}
\vspace{-0.3cm}
\scriptsize
\begin{tabular}{lcccc}\hline
\toprule
\bfseries Classifier & \bfseries Precision & \bfseries Recall & \bfseries F-measure & \bfseries PR-AUC  \\
\midrule
Random Forest & \textbf{0.83} & 0.78 & 0.81 & \textbf{0.86}\\
Support Vector Machine & 0.78 & 0.74 & 0.76 & \textbf{0.86}\\
Naive Bayes & 0.72 & 0.46 & 0.56 & 0.72\\
Logistic Regression & 0.73 & 0.70 & 0.71& 0.79\\
\textbf{Convolutional Neural Network} & 0.82 & \textbf{0.82} & \textbf{0.82} & \textbf{0.86}
 \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-0.4cm}
\end{table}

